Second Order QED Processes in an Intense Electromagnetic Field

Some non linear, second order QED processes in the presence of intense plane electromagnetic waves are investigated. Analytic expressions with general kinematics are derived for Compton scattering and $e^+e^-$ pair production in a circularly polarised external electromagnetic field. The differential cross sections were investigated numerically for photon energies up to 50 MeV, external field intensity parameter $\nu^2$ to value 2, and all scattering angles. The variation of full cross sections with respect to external field intensity was also established. The presence of the external field led to resonances in the Compton scattering and pair production differential cross sections. These resonances were investigated by calculating the electron self energy in the presence of the external field. At resonance the differential cross sections were enhanced by several orders of magnitude. The resonances occurred for values of external field intensity parameter $\nu^2 <1$, lowering the limit of $\nu^2 \sim 1$ at which point non linear effects in first order external field QED processes become important. Generally, full cross sections increased with increasing external field intensity, though peaking sharply for Compton scattering and levelling off for pair production. An application was made to non linear background studies at $e^+e^-$ linear colliders. The pair production process and electron self energy were studied for the case of a constant crossed electromagnetic field. It was found that previous analytic expressions required the external field to be azimuthally symmetric. New analytic expressions for the more general non azimuthally symmetric case were developed and a numerical parameter range equivalent to that proposed for future linear collider designs was considered.

==> tex/tables/c_allfig.tex <==
\LaTeXparent{thesis.tex}

%--------------------------------------------------------------
\section{Stimulated Compton scattering figures} 
%--------------------------------------------------------------

Throughout this chapter, the particle directions will be specified by 
the notation: $(\mbox{Polar angle},$ $\mbox{Azimuthal angle})$,
with respect to the optical axis coordinate system. In addition, the symbol $\alpha$ will
represent the aperture angle and the symbol $k_{f}$ will represent the laser
photon energy. 

\begin{table}[t]
\begin{tabular}{|l|l|l|l|l|} \hline
$k_{F}$(MeV) & $|{\vb k}|$(MeV) & $\hat{{\vb k}}$ & $\hat{{\vb p}}^{+}$ & figure(s) \\ \hline
1 & 10 & (45$^{\circ}$,0$^{\circ}$) & (0$^{\circ}\rightarrow$90$^{\circ}$,0$^{\circ}$) & \ref{ngraph6} \\ \cline{4-5}
  &    &          & (0$^{\circ}\rightarrow$90$^{\circ}$,0$^{\circ}\rightarrow$20$^{\circ}$) & \ref{ngraph7}, \ref{ngraph8} \\ \cline{3-5}
  &    & (90$^{\circ}$,0$^{\circ}$) & (0$^{\circ}\rightarrow$180$^{\circ}$,0$^{\circ}$) & \ref{ngraph9} \\ \cline{4-5}
  &    &          & (0$^{\circ}\rightarrow$180$^{\circ}$,0$^{\circ}\rightarrow$20$^{\circ}$) & \ref{ngraph10}, \ref{ngraph11} \\ \cline{3-5}
  &    & (45$^{\circ}$,90$^{\circ}$) & (0$^{\circ}\rightarrow$90$^{\circ}$,90$^{\circ}$) & \ref{ngraph12} \\ \cline{4-5}
  &    &          & (0$^{\circ}\rightarrow$180$^{\circ}$,90$^{\circ}\rightarrow$110$^{\circ}$) & \ref{ngraph13}, \ref{ngraph14} \\ \cline{3-5}
  &    & (180$^{\circ}$,0$^{\circ}$) & (0$^{\circ}\rightarrow$360$^{\circ}$,0$^{\circ}$) &  \ref{pp210} \\ \cline{4-5}
  &    &          & (0$^{\circ}\rightarrow$360$^{\circ}$,90$^{\circ}$) & \ref{pp310} \\ \hline
1 & 5  & (45$^{\circ}$,0$^{\circ}$) & (0$^{\circ}\rightarrow$90$^{\circ}$,0$^{\circ}$) & \ref{ngraph1}, \ref{ngraph17} \\ \cline{3-5}
  &    & (90$^{\circ}$,0$^{\circ}$) & (0$^{\circ}\rightarrow$180$^{\circ}$,0$^{\circ}$) & \ref{ngraph2} \\ \cline{3-5}
  &    & (90$^{\circ}$,90$^{\circ}$) & (0$^{\circ}\rightarrow$180$^{\circ}$,90$^{\circ}$) & \ref{ngraph3} \\ \cline{3-5}
  &    & (45$^{\circ}$,90$^{\circ}$) & (0$^{\circ}\rightarrow$90$^{\circ}$,90$^{\circ}$) & \ref{ngraph4} \\ \cline{3-5}
  &    & (180$^{\circ}$,0$^{\circ}$) & (0$^{\circ}\rightarrow$360$^{\circ}$,0$^{\circ}$) & \ref{pp45} \\ \cline{4-5}
  &    &          & (0$^{\circ}\rightarrow$360$^{\circ}$,90$^{\circ}$) & \ref{pp55} \\ \hline
1 &100 & (45$^{\circ}$,0$^{\circ}$) & (44.6$^{\circ}\rightarrow$45.4$^{\circ}$,0$^{\circ}$) &  \ref{ngraph15} \\ \hline
10 & 10 & (45$^{\circ}$,0$^{\circ}$) & (-20$^{\circ}\rightarrow$60$^{\circ}$,0$^{\circ}$) & \ref{ngraph30}, \ref{ngraph31} \\ \hline
\end{tabular}
\caption{The scattering geometries and energy regimes which are investigated 
in the present section for the stimulated compton scattering differential 
cross section.} 

%\label{tabppdtr}
\end{table}

\subsection{Compton differential cross sections} 
\subsubsection{Plots vs L}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_l/varv2/data5.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_l/varv2/data5.ps \\
wi=0.08, w=0.1, theti=0, phi=0, thetf=45}
%\label{ngraph7}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_l/varv2/data1a.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_l/varv2/data1a.ps \\
wi=0.0008, w=0.001, theti=10, phi=0, thetf=45}
%\label{ngraph7}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_l/varv2/data2a.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_l/varv2/data2a.ps \\
wi=2E-6, w=2.3E-6, theti=10, phi=0, thetf=45}
%\label{ngraph7}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_l/varv2/data3a.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_l/varv2/data3a.ps \\
wi=0.015, w=0.001, theti=10, phi=0, thetf=45}
%\label{ngraph7}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_l/varv2/data4a.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_l/varv2/data4a.ps \\
wi=0.0015, w=0.001, theti=10, phi=0, thetf=45}
%\label{ngraph7}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_l/varv2/data4b.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_l/varv2/data4b.ps \\
wi=0.0015, w=0.001, theti=45, phi=0, thetf=45}
%\label{ngraph7}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_l/run1.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_l/run1.ps \\
v2=0.1, w=0.001, theti=45, phi=0, thetf=45}
%\label{ngraph7}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_l/run2.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_l/run2.ps \\
v2=0.1, wi=0.0015, theti=45, phi=0, thetf=45}
%\label{ngraph7}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_l/run3.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_l/run3.ps \\
v2=0.1, wi=0.0015, w=0.001, phi=0, thetf=45}
%\label{ngraph7}
\end{figure}

\clearpage

\subsubsection{Plots vs thetf}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_thetf/v2.442/data1.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_thetf/v2.442/data1.ps \\
v2=0.442, wi=9.79E-5, w=9.79E-6, phi=0}
%\label{ngraph6}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_thetf/v2.442/data2.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_thetf/v2.442/data2.ps \\
v2=0.442, wi=9.79E-7, w=9.79E-6, phi=0}
%\label{ngraph7}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_thetf/v2.442/data3.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_thetf/v2.442/data3.ps \\
v2=0.442, wi=9.9E-6, w=9.79E-6, phi=0}
%\label{ngraph8}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_thetf/v2.162/data1.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_thetf/v2.162/data1.ps \\
v2=0.162, wi=2.3E-5, w=2.3E-6, phi=0}
%\label{ngraph8}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_thetf/v2.1/run1.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_thetf/v2.1/run1.ps \\
v2=0.1, wi=0.0015, w=0.001, phi=0}
%\label{ngraph8}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/initdata/thetivar/runs3a.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/initdata/thetivar/runs3a.ps \\
v2=0.1, wi=0.08, w=0.1, phi=0}
%\label{ngraph8}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/initdata/thetf/thetf1.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/initdata/thetf/thetf1.ps \\
wi=0.08, w=0.1, theti=10, phi=0}
%\label{ngraph8}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_thetf/varv2/run1.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_thetf/varv2/run1.ps \\
wi=0.0015, w=0.001, theti=45, phi=0}
%\label{ngraph8}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_thetf/varv2/run2.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_thetf/varv2/run2.ps \\
wi=0.0015, w=0.001, theti=90, phi=0}
%\label{ngraph8}
\end{figure}

\subsubsection{Plots vs v2}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/diffdata/vs_v2/run2.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/diffdata/vs\_v2/run2.ps \\
wi=0.0015, w=0.001, theti=90, phi=0}
%\label{ngraph8}
\end{figure}

\clearpage

\subsection{Compton total cross section} 

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/crosdata/vs_l/data1.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/crosdata/vs\_l/data1.ps \\
v2=0.5, wi=0.0008, w=0.001, theti=?, phi=0}
%\label{ngraph20}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/crosdata/vs_theti/data1.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/crosdata/vs\_theti/data1.ps \\
v2=0.1, wi=0.0008, w=0.001, theti=?, phi=0}
%\label{ngraph20}
\end{figure}

\begin{figure}
 \centerline{\psfig{figure=c:/thesis/compton/crosdata/vs_theti/data2.ps,height=8cm,width=10cm}}
\caption{c:/thesis/compton/crosdata/vs\_theti/data2.ps \\
v2=0.1, wi=0.0015, w=0.001, theti=?, phi=0}
%\label{ngraph20}
\end{figure}


